Page Segmentation using Visual Adjacency Analysis

Page segmentation is a web page analysis process that divides a page into cohesive segments, such as sidebars, headers, and footers. Current page segmentation approaches use either the DOM, textual content, or rendering style information of the page. However, these approaches have a number of drawbacks, such as a large number of parameters and rigid assumptions about the page, which negatively impact their segmentation accuracy. We propose a novel page segmentation approach based on visual analysis of localized adjacency regions. It combines DOM attributes and visual analysis to build features of a given page and guide an unsupervised clustering. We evaluate our approach on 35 real-world web pages, and examine the effectiveness and efficiency of segmentation. The results show that, compared with state-of-the-art, our approach achieves an average of 156% increase in precision and 249% improvement in F-measure.

==> figures/intro-stats.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[t]{.44\textwidth}
  % \begin{figure}[b]
    \centering
    \includegraphics[width=0.88\columnwidth,height=6cm]{figures/population-plot}
    % \hspace{1cm}
    \caption{Number of people with accessibility impairments (vision, hand control, cognitive, or hearing) in the United States
    and the European Union. To put the numbers in perspective, the number of people with impairment is
    comparable to the population of entire countries. (Sourced from: \cite{stats:accessibility_population:US, stats:accessibility_population:EU})}
    \label{fig:population-plot}
  % \end{figure}
  \end{minipage}
  \hspace{1cm}
  \begin{minipage}[t]{.44\textwidth}
  % \hfill
  % \begin{figure}[b]
    \centering
    \includegraphics[width=0.88\columnwidth]{figures/lawsuits-plot}
    \caption{Number of web accessibility lawsuits filed in US federal courts per year. The number of lawsuits increased by around \%3800 over the four-year period 2015-2018. (Sourced from: \cite{stats:accessibility_lawsuits:US_1, stats:accessibility_lawsuits:US_2})}
    \label{fig:lawsuits-plot}
  % \end{figure}
  \end{minipage}
  \end{figure*}

